Improving Utility for Privacy-Preserving Analysis of Correlated Columns using Pufferfish Privacy

Surveys are an important tool for many areas of social science research, but privacy concerns can complicate the collection and analysis of survey data. Differentially private analyses of survey data can address these concerns, but at the cost of accuracy - especially for high-dimensional statistics. We present a novel privacy mechanism, the Tabular DDP Mechanism, designed for high-dimensional statistics with incomplete correlation. The Tabular DDP Mechanism satisfies dependent differential privacy, a variant of Pufferfish privacy; it works by building a causal model of the sensitive data, then calibrating noise to the level of correlation between statistics. An empirical evaluation on survey data shows that the Tabular DDP Mechanism can significantly improve accuracy over the Laplace mechanism.

==> old.tex <==
\subsection{Privacy Definition}


We define attribute differential privacy (ADP) as a relaxation of
$\epsilon$-differential privacy. ADP relaxes the \emph{distance
  metric} on pairs of databases. The ``standard'' distance metric on a
pair of databases measures the \emph{number of rows on which they
  differ}; the distance metric for ADP instead measures the
\emph{number of attributes on which they differ}.

\begin{definition}[Distance metric for ADP]
  The distance between two databases $D_1$ and $D_2$ under attribute
  differential privacy (ADP) is:
  %
  \[d_{ADP}(D_1, D_2) = \sum_{c \in cols} \lVert D_1[c] - D_2[c] \rVert_1\]
  \label{def:distance_metric}
\end{definition}

\noindent The formal definition of attribute differential privacy is
the same as the definition of differential privacy, but uses the
distance metric $d_{ADP}$.

\begin{definition}[Attribute Differential Privacy (ADP)]
  A randomized mechanism $\mathcal{M}: \mathcal{D} \rightarrow
  \mathbb{R}^k$ satisfies $\epsilon$-attribute differential privacy
  ($\epsilon$-ADP) if for all neighboring databases $D_1$ and $D_2$
  such that $d_{ADP}(D_1, D_2) \leq 1$, and all possible sets of
  outcomes $O$:
  %
  \[ \Pr[\mathcal{M}(D_1) \in O] \leq
    \exp(\epsilon) \cdot \Pr[\mathcal{M}(D_2) \in O]\]
\end{definition}

The implication of this definition is that our privacy guarantee no
longer protects the \emph{presence or absence of an individual} in the
data, but rather the \emph{presence or absence of a single attribute}
in the data. These two guarantees are clearly not interchangeable!
However, in many contexts, privacy harm to individuals comes not from
the disclosure of their participation, but from the disclosure of
their sensitive attributes in the underlying data. ADP is designed to
provide higher accuracy statistics in this common context.

\subsection{ADP for Monty Hall}

As an example of the ADP guarantee, consider the data collected from
Monty Hall games appearing in Figure~\ref{fig:monty_data}. ADP
protects the values of \emph{attributes} in this data, rather than the
presence or absence of whole \emph{rows}. An ADP mechanism for
answering queries over this data may reveal that a game took place,
but should not reveal any of the individual attributes associated with
that game.

This goal is reflected in the distance metric for databases
(Definition~\ref{def:distance_metric}). The distance metric says that
two databases of Monty Hall games are neighbors if they differ in one
attribute. Databases that differ in more than one
attribute---including those that differ in whole rows---are not
neighbors. Unlike in differential privacy, adding or removing a row
does not produce a neighboring database.

Achieving ADP is challenging, due to the possible correlations between
attributes. The Bayesian network in Figure~\ref{fig:bayesian_network}
tells us that we can release statistics about the first two columns
using parallel composition, because they are conditionally
independent. For example, we might release noisy histograms over the
``Prize Door'' and ``First Selection'' columns; we can add Laplace
noise scaled to $\frac{1}{\epsilon}$ to each histogram and achieve
$\epsilon$-ADP \emph{in total}, by parallel composition.

If we would also like to release a histogram over the ``Monty Opens''
column, then our accounting task becomes more complicated: this column
is \emph{not} conditionally independent of the others. In standard
$\epsilon$-differential privacy, we would use sequential composition.
Under attribute differential privacy, when the dependence is not
\emph{fully} conditional (i.e. with probability 1), as in the Monty
Hall problem, we can bound the privacy loss more tightly using the
mechanism proposed in Section~\ref{sec:adp-mech}.

\section{An ADP Mechanism for Counting Queries}
\label{sec:adp-mech}


\paragraph{Problem setup.}
We have two columns, $A$ and $B$. Each has a domain of values $dom(a)
= \mathcal{A}$ and $dom(b) = \mathcal{B}$. Let $Q_A$ and $Q_B$ be
linear counting queries over the two columns (e.g. parts of a
histogram query, that count after filtering). Let $L(\cdot)$ be the
Laplace mechanism.

\subsection{Dependent Sensitivity}

\begin{definition}[Dependent sensitivity]
  Let $f_A : \mathcal{A} \rightarrow \mathbb{R}^k$ be a query over
  attribute $A$ with $L_1$ sensitivity of 1. Let $C_1, \dots, C_k$ be
  the attributes that $A$ conditionally depends on. The
  \emph{dependent $L_1$ sensitivity} of $f$ is:
  % 
  \[\max_{a, a' \in \mathcal{A}} \max_{c_1, \dots, c_k \in \mathcal{C_1}, \dots, \mathcal{C_1}}
    \frac{\Pr[a \mid c_1, \dots, c_k ]}
    {\Pr[a' \mid c_1, \dots, c_k ]} \]
\end{definition}

When the set of dependencies $c_1, \dots, c_k$ is empty (i.e. the
attribute $A$ is independent), then the dependent sensitivity is 1, as
expected. \jn{not sure about this, need to check}

\begin{definition}[Laplace Mechanism for ADP]
  Let $f_A : \mathcal{A} \rightarrow \mathbb{R}$ be a query over
  attribute $A$ with dependent sensitivity $s$. The following
  mechanism satisfies $\epsilon$-ADP:
  %
  \[F_A(D) = f_A(D[A]) + \textsf{Lap}\Big(\frac{s}{\epsilon}\Big)\]
  %
  where $\textsf{Lap}(\sigma)$ is a draw from a Laplace distribution with mean
  0 and scale $\sigma$.
  \label{def:laplace_mech}
\end{definition}

\noindent It is no surprise that we can define the Laplace mechanism
for ADP; this definition also satisfies $\epsilon$-differential
privacy, and provides no utility benefit. In the next section, we will
define a parallel version of the mechanism that yields better utility.

\subsection{Parallel Laplace Mechanism}

Consider two queries $f_A$ and $f_B$, sensitivity-1 queries on
attributes $A$ and $B$ respectively. Releasing both query results
under $\epsilon$-differential privacy requires sequential composition.
Under ADP, we can apply the \emph{Parallel Laplace Mechanism}.

\begin{definition}[Parallel Laplace Mechanism]
  Let $f_A : \mathcal{A} \rightarrow \mathbb{R}$ and $f_B :
  \mathcal{B} \rightarrow \mathbb{R}$ be queries over attribute
  $A$ and $B$ respectively. Let $s_A$ be the dependent sensitivity of
  $f_A$, and $s_B$ be the dependent sensitivity of $f_B$. The
  following mechanism satisfies $\epsilon$-ADP:
  %
  \[F_{A,B}(D) =
    \Big(f_A(D[A]) + \textsf{Lap}\Big(\frac{s_A}{\epsilon}\Big),
    f_B(D[B]) + \textsf{Lap}\Big(\frac{s_B}{\epsilon}\Big)\Big)\]
  \label{def:laplace_mech_parallel}
\end{definition}

\noindent Under sequential composition, the privacy cost would be
$2\epsilon$; as we will see later, the savings in privacy cost gets
\emph{better} as the number of attributes increases. This kind of
parallel composition is impossible under $\epsilon$-differential
privacy, and is the key factor behind the increased utility possible
under ADP.

\begin{theorem}[Privacy of the Parallel Laplace mechanism]
  The parallel Laplace mechanism for ADP
  (Definition~\ref{def:laplace_mech_parallel}) satisfies
  $\epsilon$-ADP.
\end{theorem}

\begin{proof}
  \jn{TODO: proof sketch}
  
\begin{align*}
  &\max_{A, A', B}
    \frac{\Pr[L(Q_A(A)) = \hat{c_a}, L(Q_B(B)) = \hat{c_b} ]}
    {\Pr[L(Q_A(A')) = \hat{c_a}, L(Q_B(B)) = \hat{c_b} ]} & \text{def. of privacy}\\
  = &\max_{A, A'}
    \frac{\Pr[L(Q_A(A)) = \hat{c_a} ] \sum_{B} \Pr[L(Q_B(B)) = \hat{c_b}] \Pr[Q_B(B) \mid A]}
      {\Pr[L(Q_A(A')) = \hat{c_a} ] \sum_{B} \Pr[L(Q_B(B)) = \hat{c_b}] \Pr[Q_B(B) \mid A']}
                                                         & \text{law total prob.}\\
  \leq &\max_{A, A'}
         \frac{\Pr[L(Q_A(A)) = \hat{c_a} ]}
         {\Pr[L(Q_A(A')) = \hat{c_a} ]} \cdot
         \max_{A, A'}
         \frac{\sum_{B} \Pr[L(Q_B(B)) = \hat{c_b}] \Pr[B \mid A]}
         {\sum_{B} \Pr[L(Q_B(B)) = \hat{c_b}] \Pr[B \mid A']}
                                                         & \text{loose upper bound}\\
  \leq & \exp(\epsilon) \cdot
         \max_{A, A'}
         \frac{\sum_{B} \Pr[L(Q_B(B)) = \hat{c_b}] \Pr[B \mid A]}
         {\sum_{B} \Pr[L(Q_B(B)) = \hat{c_b}] \Pr[B \mid A']}
                                                         & \text{def. Laplace mech.}\\
  \leq & \exp(\epsilon) \cdot
      \max_{A, A'} \max_B
      \frac{\Pr[L(Q_B(B)) = \hat{c_b}] \Pr[B \mid A]}
      {\Pr[L(Q_B(B)) = \hat{c_b}] \Pr[B \mid A']}& \text{loose upper bound}\\
  = & \exp(\epsilon) \cdot
      \max_{A, A'} \max_B
      \frac{\Pr[B \mid A]}
      {\Pr[B \mid A']}& \text{cancel}\\
  = & \log \Big(\epsilon +
      \max_{A, A'} \max_B
      \frac{\Pr[B \mid A]}
      {\Pr[B \mid A']}\Big)& \text{log rule}\\
\end{align*}
\end{proof}

\begin{figure}
  \centering
  {%\footnotesize
  \begin{tabular}{l l ||l l l}
    Prize & First & MO & MO & MO \\
    & Select. & =1 & =2 & =3 \\
    \hline \hline
    Door 1 &	Door 1 &	0 &	$\frac{1}{2}$ &	$\frac{1}{2}$ \\
    Door 1 &	Door 2 &	0 &	0 &	1 \\
    Door 1 &	Door 3 &	0 &	1 &	0 \\
    Door 2 &	Door 1 &	0 &	0 &	1 \\
    Door 2 &	Door 2 &	$\frac{1}{2}$ &	0& 	$\frac{1}{2}$ \\
    Door 2 &	Door 3 &	1 &	0& 	0 \\
    Door 3 &	Door 1 &	0 &	1& 	0 \\
    Door 3 &	Door 2 &	1 &	0& 	0 \\
    Door 3 &	Door 3 &	$\frac{1}{2}$& 	$\frac{1}{2}$& 	0 \\
  \end{tabular}}
  \caption{Conditional Probability Table, Monty Hall Problem.}
\end{figure}

\paragraph{Example: parallel ADP for Monty Hall.}
We now apply the parallel Laplace mechanism for ADP to the Monty Hall
problem defined earlier. For simplicity of presentation, we will
release counts for only the ``first selection'' and ``Monty opens''
attributes.

\begin{proposition}
  Releasing the following two values satisfies a \emph{total} of
  $\epsilon$-ADP:

  \begin{enumerate}
  \item $Q_{\text{First Selection} = 1}(D) + \textsf{Lap}\Big(\frac{s_1}{\epsilon}\Big)$
  \item $Q_{\text{Monty Opens} = 1}(D) + \textsf{Lap}\Big(\frac{s_2}{\epsilon}\Big)$
  \end{enumerate}
\end{proposition}

\begin{proof}
  We need to show that:
  %
  \[\max_{D, D'} \frac{\Pr[L(Q_A(D)) = \hat{c_a}, L(Q_B(D)) = \hat{c_b} ]}
    {\Pr[L(Q_A(D')) = \hat{c_a}, L(Q_B(D)) = \hat{c_b} ]}\]

  Under the distance metric for ADP, there are two cases: either
  attribute $A$ changes (``first selection'') or attribute $B$ changes
  (``Monty opens'').

  \paragraph{Case 1: attribute $A$ changes.}
  We need to show that:
  %
  \[\max_{A, A', B} \frac{\Pr[L(Q_A(A)) = \hat{c_a}, L(Q_B(B)) = \hat{c_b} ]}
    {\Pr[L(Q_A(A')) = \hat{c_a}, L(Q_B(B)) = \hat{c_b} ]}\]
  
  \paragraph{Case 2: attribute $B$ changes.}
  We need to show that:
  %
  \[\max_{A, B, B'} \frac{\Pr[L(Q_A(A)) = \hat{c_a}, L(Q_B(B)) = \hat{c_b} ]}
    {\Pr[L(Q_A(A)) = \hat{c_a}, L(Q_B(B')) = \hat{c_b} ]}\]
\end{proof}

\jn{I'm stuck here}


\section{An ADP Mechanism for Histograms}


